Specformer: Spectral Graph Neural Networks Meet Transformers

Spectral graph neural networks (GNNs) learn graph representations via spectral-domain graph convolutions. However, most existing spectral graph filters are scalar-to-scalar functions, i.e., mapping a single eigenvalue to a single filtered value, thus ignoring the global pattern of the spectrum. Furthermore, these filters are often constructed based on some fixed-order polynomials, which have limited expressiveness and flexibility. To tackle these issues, we introduce Specformer, which effectively encodes the set of all eigenvalues and performs self-attention in the spectral domain, leading to a learnable set-to-set spectral filter. We also design a decoder with learnable bases to enable non-local graph convolution. Importantly, Specformer is equivariant to permutation. By stacking multiple Specformer layers, one can build a powerful spectral GNN. On synthetic datasets, we show that our Specformer can better recover ground-truth spectral filters than other spectral GNNs. Extensive experiments of both node-level and graph-level tasks on real-world graph datasets show that our Specformer outperforms state-of-the-art GNNs and learns meaningful spectrum patterns. Code and data are available at https://github.com/bdy9527/Specformer.

==> iclr2023/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/background.tex <==
\section{Background}

In this section, we introduce some preliminaries of graph signal processing (GSP) \citep{GSP1} and Transformer \citep{transformer}.

\paragraph{Preliminary.}
Assume that we have a graph $\gG=(\gV, \gE)$, where $\gV$ denotes the node set with $|\gV|=n$ and $\gE$ is the edge set.
The corresponding adjacency matrix $\mA \in \{0,1\}^{n \times n}$, where $\emA_{ij}=1$ if there is an edge between nodes $i$ and $j$, and $A_{ij} =0$ otherwise.
% \lele{[If the adjacency matrix only takes binary values, we can simplify the range to $\mA \in \{0,1\}^{n \times n}$]} 
The normalized graph Laplacian matrix is defined as $\mL=\mI_{n}-\mD^{-1/2} \mA \mD^{-1/2}$, where $\mI_{n}$ is the $n\times n$ identity matrix and $\mD$ is the diagonal degree matrix with diagonal entries $\emD_{ii}=\sum_{j} \emA_{ij}$ for all $i \in \mathcal{V}$ and off-diagonal entries $D_{ij} = 0$ for $i \neq j$.
We assume $\gG$ is undirected.
% \lele{[Do we ever consider any asymmetric adjacency matrix in this paper? If not, we can use ``'' instead of ``generally''.]}
Hence, $\mL$ is a real symmetric matrix, whose spectral decomposition can be written as $\mL = \mU \mLambda \mU^{\top}$, where the columns of $\mU$ are the eigenvectors and $\mLambda = \text{diag} ( [\lambda_{1},\lambda_{2},\dots,\lambda_{n}] )$ are the corresponding eigenvalues ranged in $[0, 2]$. 

\paragraph{Graph Signal Processing (GSP).}
Spectral GNNs rely on several important concepts from GSP, namely, spectral filtering, graph Fourier transform and its inverse.
The graph Fourier transform is written as $\hat{\vx}=\mU^{\top} \vx$, where $\vx \in \mathbb{R}^{n \times 1}$ is a graph signal and $\hat{\vx} \in \R^{n \times 1}$ represents the Fourier coefficients.
Then a spectral filter $G_{\theta}$ is used to scale $\hat{\vx}$. 
Finally, the inverse graph Fourier transform is applied to yield the filtered signal in spatial domain $\tilde{\vx}=\mU G_{\theta} \hat{\vx}$. 
The key task in GSP is to design a powerful spectral filter $G_{\theta}$ so that we can exploit the useful frequency information.
% \lele{[Is it better to write $G_\theta(\hat{\vx})$? Right now, $\tilde{\vx}=\mU G_{\theta} \hat{\vx}$ reads like matrix multiplication.]}

\paragraph{Transformer.} Transformer is a powerful deep learning model, which is widely used in natural language processing \citep{BERT}, vision \citep{ViT}, and graphs \citep{Graphormer, GPS}.
Each Transformer layer consists of two components: a multi-head self-attention (MHA) module and a token-wise feed-forward network (FFN).
Given the input representations $\mH=[\vh_{1}^{\top},\dots,\vh_{n}^{\top}]\in \mathbb{R}^{n \times d}$, where $d$ is the hidden dimension, MHA first projects $\mH$ into query, key and value through three matrices ($\mW^{Q}$, $\mW^{K}$ and $\mW^{V}$) to calculate attentions. And FFN is then used to add transformation. The model can be written as follows where we denote the query dimension as $d_q$.
For simplicity, we omit the bias and the description of multi-head attention.
\begin{equation}
\begin{split}
\text{Attention}(\mQ, \mK, \mV)= \text{Softmax} (\frac{\mQ \mK^{\top}}{\sqrt{d_{q}}})\mV, \\
    \mQ=\mH\mW^{Q}, \ \mK=\mH\mW^{K}, \ \mV=\mH\mW^{V}.
\end{split}
\end{equation}

==> sections/conclusion.tex <==
\section{Conclusion}
\vspace{-5pt}
In this paper, we propose Specformer that leverages Transformer to build a set-to-set spectral filter along with learnable bases.
Specformer effectively captures magnitudes and relative dependencies of the eigenvalues in a permutation-equivariant fashion and can perform non-local graph convolution.
Experiments on synthetic and real-world datasets demonstrate that Specformer outperforms various GNNs and learns meaningful spectrum patterns.
A promising future direction is to improve the efficiency of Specformer through sparsifying the self-attention matrix of Transformer.

==> sections/exp.tex <==
\section{Experiments}
\vspace{-5pt}
In this section, we conduct experiments on a synthetic dataset and a wide range of real-world graph datasets to verify the effectiveness of our Specformer.
% and compare the performance of Specformer and other state-of-the-art methods in diverse tasks.
% , including node classification, graph classification, and graph regression.

\begin{table}[t]
  \centering
  \caption{Node regression results, mean of the sum of squared error \& $R^{2}$ score, on synthetic data.}
  \resizebox{0.95\linewidth}{!}{
    \begin{tabular}{lccccc}
    \toprule
        \multicolumn{1}{c}{\multirow{2}[4]{*}{\makecell[c]{\textbf{Model}\\($\sim$\textbf{2k param.})}}} &
        \multicolumn{1}{c}{\textbf{Low-pass}} & \multicolumn{1}{c}{\textbf{High-pass}} & \multicolumn{1}{c}{\textbf{Band-pass}} & \multicolumn{1}{c}{\textbf{Band-rejection}} & \multicolumn{1}{c}{\textbf{Comb}}\\
\cmidrule(lr){2-6}  & \begin{small} $\exp(-10 \lambda^{2})$ \end{small} 
& \begin{small} $1 - \exp(-10 \lambda^{2})$ \end{small}
& \begin{small} $\exp(-10 (\lambda - 1)^{2})$ \end{small} 
& \begin{small} $1 - \exp(-10 (\lambda - 1)^{2})$ \end{small} 
& \begin{small} $\left| \sin(\pi \lambda) \right|$ \end{small} \\
    \midrule
    GCN         & 3.4799(.9872) & 67.6635(.2364) & 25.8755(.1148) & 21.0747(.9438) & 50.5120(.2977) \\
    GAT         & 2.3574(.9905) & 21.9618(.7529) & 14.4326(.4823) & 12.6384(.9652) & 23.1813(.6957) \\
    ChebyNet    & 0.8220(.9973) & 0.7867(.9903) & 2.2722(.9104) & 2.5296(.9934) & 4.0735(.9447) \\
    GPR-GNN     & 0.4169(.9984) & 0.0943(.9986) & 3.5121(.8551) & 3.7917(.9905) & 4.6549(.9311) \\
    BernNet     & 0.0314(.9999) & 0.0113(.9999) & 0.0411(.9984) & 0.9313(.9973) & 0.9982(.9868) \\
    JacobiConv  & 0.0003(.9999) & 0.0064(.9999) & 0.0213(.9999) & 0.0156(.9999) & 0.2933(.9995) \\
    Specformer  & \textbf{0.0002(.9999)} & \textbf{0.0026(.9999)} & \textbf{0.0017(.9999)} & \textbf{0.0014(.9999)} & \textbf{0.0057(.9999)} \\
    \bottomrule
    \end{tabular}}%
    \label{tab:toy_regression}%
    \vspace{-5pt}
\end{table}%

\begin{figure}[t]
    \centering
    \subfigure[High-pass]{
        \includegraphics[width=0.3\linewidth]{pic/high.pdf}
    }
    \subfigure[Band-rejection]{
        \includegraphics[width=0.3\linewidth]{pic/rej.pdf}
    }
    \subfigure[Comb]{
        \includegraphics[width=0.3\linewidth]{pic/comb.pdf}
    }
    \vspace{-6pt}
    \caption{Illustrations of filters learned by two polynomial GNNs and Specformer.}
    \label{fig:toy_filter}
    \vspace{-6pt}
\end{figure}

\subsection{Learning Spectral Filters on Synthetic Data}

% We first test whether our Specformer can learn the pre-defined spectral filters on synthetic data.
% demonstrate the effectiveness of Specformer with some synthetic graphs.
% Specifically, we aim to test whether spectral-based GNNs can learn the pre-defined filters well.

\vspace{-5pt}
\paragraph{Dataset description.} We take 50 images with the resolution of 100$\times$100 from the Image Processing Toolbox \footnote{https://ww2.mathworks.cn/products/image.html}. Each image is processed as a 2D regular 4-neighborhood grid graph, and the values of pixels are the node features. Therefore, these images share the same adjacency matrix $\mA \in \R^{10000 \times 10000}$ and the $m$-th image has its graph signal $\vx_{m} \in \R^{10000 \times 1}$. Five predefined graph filters are used to generate ground truth graph signals. For example, if we use the low-pass filter with $G_{\theta} = \exp (-10 \lambda^{2})$, the filtered graph signal is calculated by $\tilde{\vx}_{m}=\mU \text{diag}[\exp (-10 \lambda^{2}_{1}), \dots, \exp (-10 \lambda^{2}_{n})] \mU^{\top}\vx_{m}$.

\vspace{-10pt}
\paragraph{Setup.} We choose six Spectral GNNs as baselines: GCN \citep{GCN}, GAT \citep{GAT}, ChebyNet \citep{ChebyNet}, GPR-GNN \citep{GPR-GNN}, BernNet \citep{BernNet}, and JacobiConv \citep{Jacobi}.
Each method takes $\mA$ and $\vx_{m}$ as inputs, and tries to minimize the sum of squared error between the outputs $\hat{\vx}_{m}$ and the pre-filtered graph signal $\tilde{\vx}_{m}$.
We tune the number of hidden units to ensure that each method has nearly $2$K trainable parameters. The polynomial order is set to 10 for ChebyNet, GPR-GNN, and BernNet.
For our model, we use Specformer-Small with 16 hidden units and 1 head.
In training, the maximum number of epochs is set to 2000, and the model will be stopped early if the loss does not descend 200 epochs.
All regularization tricks are removed.
The learning rate is set to 0.01 for all models.
We use two metrics to evaluate each method: sum of squared error and $R^{2}$ score.

\vspace{-10pt}
\paragraph{Results.} The quantitative experiment results are shown in Table \ref{tab:toy_regression}, from which we can see that Specformer achieves the best performance on all synthetic graphs.
Especially, it has more improvements on challenging graphs, such as Band-rejection and Comb. 
This validates the effectiveness of Specformer in learning complex graph filters.
In addition, we can see that GCN and GAT only perform better on the homophilic graph, which reflects that only using low-frequency information is not enough. 
Polynomial-based GNNs, \ie, ChebyNet, GPR-GNN, BernNet, and JacobiConv, have more stable performances. 
But their expressiveness is still weaker than Specformer.
We visualize the graph filters learned by GPR-GNN, BernNet, and Specformer in Figure \ref{fig:toy_filter}, which further validates our claims.
The horizontal axis presents the original eigenvalues, and the vertical axis indicates the corresponding new eigenvalues.
For clarity, we uniformly downsample the eigenvalues at a ratio of 1:200 and only visualize three graphs because the situations of Low-pass and High-pass are similar. The same goes for Band-pass and Band-rejection.
It can be seen that all methods can fit the easy filters well, \ie, High-pass. However, the polynomial-based GNNs cannot learn the narrow bands in Band-rejection and Comb, \eg, $\lambda \in [0.75, 1.25]$, which harms their performance. 
On the contrary, Specformer fits the ground truth precisely, reflecting the superior learning ability over polynomials.
The spatial results, \ie, filtered images, can be seen in Appendix \ref{appendix: spatial}.

% Besides, we can see that compared with BernNet, GPR-GNN has a greater variance. The reason is that BernNet restricts the new eigenvalues to be positive, while GPR-GNN uses the basic polynomial, indicating that the constraints on eigenvalues can benefit the optimization of the spectral model.


\subsection{Node Classification}

\vspace{-5pt}
\paragraph{Datasets.} For the node classification task, we perform experiments on four homophilic datasets, \ie, Cora, Citeser, Amazon-Photo and ogbn-arXiv, and four heterophilic datasets, \ie, Chameleon, Squirrel, Actor and Penn94.
Penn94 \citep{Penn94} and arXiv \citep{OGBG} are two large scale datasets. 
Other datasets, provided by \citep{MUSAE, Geom-GCN}, are commonly used to evaluate the performance of GNNs on heterophilic and homophilic graphs.

\vspace{-10pt}
\paragraph{Baselines and settings.} 
We benchmark our model against a series of competitive baselines, including spatial GNNs, spectral GNNs, and graph Transformers.
For all datasets, we use the full-supervised split, \ie, 60\% for training, 20\% for validation, and 20\% for testing, as suggested in \citep{BernNet}.
All methods run 10 times and report the mean accuracy with a 95\% confidence interval.
For polynomial GNNs, we set the order of polynomials $K$ = 10. For other methods, we use a 2-layer module.
To ensure all models have similar numbers of parameters, in six small datasets, we set the hidden size $d=64$ for spatial and spectral GNNs and $d=32$ for graph Transformers and Specformer.
The total numbers of parameters on Photo dataset are shown in Table \ref{tab:node_cla_pfm}.
On two large datasets, we use truncated spectral decomposition to improve the scalability.
Based on the filters learned on the small datasets, we find that band-rejection filters are important for heterophilic datasets and low-pass filters are suitable for homophilic datasets.
See Figures \ref{fig:filter_of_citeseer} and \ref{fig:filter_of_squirrel}.
Therefore, we use eigenvectors with the smallest 3000 (low-frequency) and largest 3000 eigenvalues (high-frequency) for Penn94, and eigenvectors with the smallest 5000 eigenvalues (low-frequency) for arXiv.
We use one layer for Specformer and set $d=64$ in Penn94 and $d=512$ in arXiv for all methods, as suggested by \citep{Penn94, Chebyshev2}.
More details, \eg, optimizers, can be found in Appendix \ref{appendix: experimental details}.

\vspace{-10pt}
\paragraph{Results.}
In Table \ref{tab:node_cla_pfm}, we can find that Specformer outperforms state-of-the-art baselines on 7 out of 8 datasets and achieves 12\% relative improvement on the Squirrel dataset, which validates the superior learning ability of Specformer.
In addition, the improvement is more pronounced on heterophilic datasets than on homophilic datasets.
This is probably caused by the easier fitting of the low-pass filters in homophilic datasets.
The same phenomenon is also observed in the synthetic graphs.
An interesting observation is that the improvement on larger graphs, \eg, Actor and Photo, is less than that on smaller graphs. One possible reason is that the role of the self-attention mechanism is weakened, \ie, the attention values become uniform due to a large number of tokens.
% Therefore, promising future work is to enforce the self-attention module to focus on the most important tokens.
We notice that Specformer has a slightly higher variance than the baselines. This is because we set a large dropout rate to prevent overfitting.
On the two large graph datasets, we can see that graph Transformers are memory-consuming due to the self-attention.
On the contrary, Specformer reduces the time and space costs by using the truncated decomposition and shows better scalability than graph Transformers.
The time and space overheads are listed in Appendix \ref{appendix: overhead}.

\begin{table}[t]
  \centering
  \caption{Results on real-world node classification tasks. Mean accuracy (\%) ± 95\% confidence interval. * means re-implemented baselines. ``OOM'' means out of GPU memory.}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{l|c|cccc|cccc}
    \toprule
          & \multirow{2}[4]{*}{\makecell[c]{\textbf{Param.} \\ \textbf{on Photo}}} & \multicolumn{4}{c|}{\textbf{Heterophilic}} & \multicolumn{4}{c}{\textbf{Homophilic}} \\
\cmidrule{3-10}          &       & \textbf{Chameleon} & \textbf{Squirrel} & \textbf{Actor} & \textbf{Penn94} & \textbf{Cora}  & \textbf{Citeseer} & \textbf{Photo} & \textbf{arXiv} \\
    % \midrule
    % Nodes & - & 2,277 & 5,201 & 7,600 & 41,554 & 2,708 & 3,327 & 7,650 & 169,343 \\
    % Edges & - & 36,101 & 217,073 & 33,544 & 1,362,229 & 5,429 & 4,732 & 119,081 & 1,116,243 \\
    % Features & - & 2,325 & 2,089 & 932 & 4,814 & 1,433 & 3,703 & 745 & 128\\
    % Classes & - & 5     & 5     & 5   &  2  & 7     & 6     & 8 & 40 \\
    \midrule
    \multicolumn{10}{c}{Spatial-based GNNs} \\
    % \specialrule{0em}{3pt}{3pt}
    \midrule
    GCN         & 48K & 59.61±2.21 & 46.78±0.87 & 33.23±1.16 & 82.47±0.27 & 87.14±1.01 & 79.86±0.67 & 88.26±0.73 & 71.74±0.29 \\
    GAT         & 49K & 63.13±1.93 & 44.49±0.88 & 33.93±2.47 & 81.53±0.55 & 88.03±0.79 & 80.52±0.71 & 90.94±0.68 & 71.82±0.23 \\
    % Geom-GCN    & 17K & 60.90 & 38.14 & 31.63 & 84.93 & 75.14 & - \\
    H$_2$GCN    & 60K & 57.11±1.58 & 36.42±1.89 & 35.86±1.03 & OOM & 86.92±1.37 & 77.07±1.64 & 93.02±0.91 & OOM \\
    GCNII       & 49K  & 63.44±0.85 & 41.96±1.02 & 36.89±0.95 & 82.92±0.59 & 88.46±0.82 & 79.97±0.65 & 89.94±0.31 & 72.04±0.19 \\
    \midrule
    \multicolumn{10}{c}{Spectral-based GNNs} \\
    \midrule
    % LanczosNet* & - & - & - & - & - & - & - \\
    LanczosNet*     & 50K & 64.81±1.56 & 48.64±1.77 & 38.16±0.91 & 81.55±0.26 & 87.77±1.45 & 80.05±1.65 & 93.21±0.85 & 71.46±0.39 \\
    ChebyNet        & 48K & 59.28±1.25 & 40.55±0.42 & 37.61±0.89 & 81.09±0.33 & 86.67±0.82 & 79.11±0.75 & 93.77±0.32 & 71.12±0.22 \\
    GPR-GNN         & 48K & 67.28±1.09 & 50.15±1.92 & 39.92±0.67 & 81.38±0.16 & 88.57±0.69 & 80.12±0.83 & 93.85±0.28 & 71.78±0.18 \\
    BernNet         & 48K & 68.29±1.58 & 51.35±0.73  & 41.79±1.01 & 82.47±0.21 & 88.52±0.95 & 80.09±0.79 & 93.63±0.35 & 71.96±0.27 \\
    ChebNetII       & 48K & 71.37±1.01 & 57.72±0.59 & 41.75±1.07 & 83.12±0.22 & 88.71±0.93 & 80.53±0.79 & 94.92±0.33 & 72.32±0.23 \\
    JacobiConv      & 48K & 74.20±1.03 & 57.38±1.25 & 41.17±0.64 & 83.35±0.11 & \textbf{88.98±0.46} & 80.78±0.79 & 95.43±0.23 & 72.14±0.17 \\
    \midrule
    \multicolumn{10}{c}{Graph Transformers} \\
    \midrule
    Transformer*    & 37K & 46.39±1.97 & 31.90±3.16 & 39.95±1.64 & OOM & 71.83±1.68 & 70.55±1.20 & 90.05±1.50 & OOM \\
    Graphormer*     & 139K & 54.49±3.11 & 36.96±1.75 & 38.45±1.38 & OOM & 67.71±0.78 & 73.30±1.21 & 85.20±4.12 & OOM \\
    \midrule
    \midrule
    Specformer      & 32K & \textbf{74.72±1.29} & \textbf{64.64±0.81} & \textbf{41.93±1.04} & \textbf{84.32±0.32} & 88.57±1.01 & \textbf{81.49±0.94} & \textbf{95.48±0.32} & \textbf{72.37±0.18} \\
    \bottomrule
    \end{tabular}}%
  \label{tab:node_cla_pfm}%
  \vspace{-10pt}
\end{table}%

\subsection{Graph Classification and Regression}

\paragraph{Datasets.} We conduct experiments on three graph-level datasets with different scales.
ZINC \citep{ZINC} is a small subset of a large molecular dataset, which contains 12K graphs in total.
% and its target is to regress the contrained solubility of small molecules.
MolHIV and MolPCBA are taken from the Open Graph Benchmark (OGB) datasets \citep{OGBG}. MolHIV is a medium dataset that has nearly 41K graphs.
% and it is to predict the molecule’s fitness to inhibit HIV replication.
MolPCBA is the largest, containing 437K graphs.
% and 128 binary classification tasks.
For all datasets, nodes represent the atoms, and edges indicate the bonds.

\vspace{-5pt}
\paragraph{Baselines and Settings.} We choose popular MPNNs (GCN, GIN, and GatedGNN), graph Transformers with positional or structural embedding (SAN, Graphormer, and GPS), and other state-of-the-art GNNs (CIN, GIN-AK+, etc.) as the baselines of graph-level tasks. 
For the ZINC dataset, we tune the hyperparameters of Specformer to ensure that the total parameters are around 500K.


\begin{table}[t]
    \centering
    \caption{Results on graph-level datasets. $\downarrow$ means lower the better, and $\uparrow$ means higher the better.}
    \resizebox{0.65\linewidth}{!}{
    \begin{tabular}{lccc}
    \toprule
    \textbf{Model} & \textbf{ZINC($\downarrow$)} & \textbf{MolHIV($\uparrow$)} & \textbf{MolPCBA($\uparrow$)} \\
    \midrule
    GCN         & 0.367 ± 0.011 & 0.7599 ± 0.0119 & 0.2424 ± 0.0034\\
    GIN         & 0.526 ± 0.051 & 0.7707 ± 0.0149 & 0.2703 ± 0.0023\\
    GatedGCN    & 0.090 ± 0.001 & - & 0.267 ± 0.002\\
    CIN         & 0.079 ± 0.006 & \textbf{0.8094 ± 0.0057} & -\\
    GIN-AK+     & 0.080 ± 0.001 & 0.7961 ± 0.0119 & 0.2930 ± 0.0044\\
    GSN         & 0.101 ± 0.010 & 0.7799 ± 0.0100 & - \\
    DGN         & 0.168 ± 0.003 & 0.7970 ± 0.0097 & 0.2885 ± 0.0030\\
    PNA         & 0.188 ± 0.004 & 0.7905 ± 0.0132 & 0.2838 ± 0.0035\\
    Spec-GN     & 0.070 ± 0.002 & - & 0.2965 ± 0.0028\\
    \midrule
    SAN         & 0.139 ± 0.006 & 0.7785 ± 0.0025 & 0.2765 ± 0.0042\\
    Graphormer\tablefootnote{We retrain Graphomer on MolHIV and MolPCBA datasets without using pre-training and augmentation.}  & 0.122 ± 0.006 & 0.7640 ± 0.0022 & 0.2643 ± 0.0017 \\
    GPS         & 0.070 ± 0.004 & 0.7880 ± 0.0101 & 0.2907 ± 0.0028\\
    \midrule
    Specformer  & \textbf{0.066 ± 0.003} & 0.7889 ± 0.0124 & \textbf{0.2972 ± 0.0023} \\
    \bottomrule
    \end{tabular}}
    \label{tab:graph-level}%
\end{table}

\vspace{-5pt}
\paragraph{Results.}
We apply Specformer-Small, Medium, and Large for ZINC, MolHIV, and MolPCBA, respectively. The results are shown in Table \ref{tab:graph-level}.
It can be seen that Specformer outperforms the state-of-the-art models in ZINC and MolPCBA datasets, without using any hand-crafted features or pre-defined polynomials.
% As for the MolHIV dataset, the 
This phenomenon proves that directly using neural networks to learn the graph spectrum is a promising way to construct powerful GNNs.

% \begin{table}
% \begin{minipage}{.63\linewidth}
%     \centering
%     \caption{Results on medium-scale graph datasets. $\downarrow$ means lower the better, and $\uparrow$ means higher the better.}
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{lccc}
%     \toprule
%     \textbf{Model} & \textbf{ZINC($\downarrow$)} & \textbf{MolHIV($\uparrow$)} & \textbf{MolPCBA($\uparrow$)} \\
%     \midrule
%     GCN         & 0.367 ± 0.011 & 0.7599 ± 0.0119 & 0.2424 ± 0.0034\\
%     GIN         & 0.526 ± 0.051 & 0.7707 ± 0.0149 & 0.2703 ± 0.0023\\
%     GatedGCN    & 0.090 ± 0.001 & - & 0.267 ± 0.002\\
%     CIN         & 0.079 ± 0.006 & \textbf{0.8094 ± 0.0057} & -\\
%     GIN-AK+     & 0.080 ± 0.001 & 0.7961 ± 0.0119 & 0.2930 ± 0.0044\\
%     GSN         & 0.101 ± 0.010 & 0.7799 ± 0.0100 & - \\
%     DGN         & 0.168 ± 0.003 & 0.7970 ± 0.0097 & 0.2885 ± 0.0030\\
%     PNA         & 0.188 ± 0.004 & 0.7905 ± 0.0132 & 0.2838 ± 0.0035\\
%     Spec-GN     & 0.070 ± 0.002 & - & 0.2965 ± 0.0028\\
%     \midrule
%     SAN         & 0.139 ± 0.006 & 0.7785 ± 0.0025 & 0.2765 ± 0.0042\\
%     Graphormer  & 0.122 ± 0.006 & - & -\\
%     GPS         & 0.070 ± 0.004 & 0.7880 ± 0.0101 & 0.2907 ± 0.0028\\
%     \midrule
%     Specformer  & \textbf{0.066 ± 0.003} & 0.7889 ± 0.0124 & \textbf{0.2972 ± 0.0023} \\
%     \bottomrule
%     \end{tabular}}
%     \label{tab:graph-level}%
% \end{minipage}
% \
% \begin{minipage}{.35\linewidth}
%     % \vspace{-15pt}
%     \centering
%     \caption{Results on large-scale graph dataset PCQM4Mv2.}
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{lcc}
%     \toprule
%     \multirow{2}[4]{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{PCQM4Mv2}} \\
%     \cmidrule{2-3}          & \textbf{MAE($\downarrow$)} & \textbf{Param.}\\
%     \midrule
%     GCN         & 0.1379 & 2.0M \\
%     GCN-VN      & 0.1153 & 4.9M \\
%     GIN         & 0.1195 & 3.8M \\
%     GIN-VN      & 0.1083 & 6.7M \\
%     \midrule
%     GRPE        & 0.0890 & 46.2M \\
%     EGT         & 0.0869 & 89.3M \\
%     Graphormer  & 0.0864 & 48.3M \\
%     GPS-small   & 0.0938 & 6.2M \\
%     GPS-medium  & 0.0858 & 19.4M \\
%     % Spec-GN     &  &  \\
%     \midrule
%     Specformer-S  & 0.0903 & 2.7M \\
%     Specformer-M  &        & 6.4M \\
%     Specformer-L  &        & 10.1M \\
%     \bottomrule
%     \end{tabular}}
%     \label{tab:pcqm}%
% \end{minipage}
% \end{table}

\subsection{Ablation Studies}

\begin{table}[t]
    \centering
    \caption{Ablation studies on node-level and graph-level tasks.}
    \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{cccccccc}
    \toprule
    \multicolumn{2}{c}{\textbf{Encoder}} & \multicolumn{3}{c}{\textbf{Decoder}} & \multicolumn{2}{c}{\textbf{Node-level}} & \multicolumn{1}{c}{\textbf{Graph-level}} \\
    \cmidrule(lr){1-2} \cmidrule(lr){3-5} \cmidrule(lr){6-7} \cmidrule(lr){8-8}
    $\mathbf{\rho(\lambda)}$ & \textbf{Attention} & \textbf{Small} & \textbf{Medium} & \textbf{Large} & \textbf{Squirrel ($\uparrow$)} & \textbf{Citeseer ($\uparrow$)} & \textbf{MolPCBA ($\uparrow$)}\\
    \midrule
      &   &   & \Checkmark &   & 33.05 & 80.57 & 0.2696 \\
    \Checkmark &   &   & \Checkmark &   & 63.78 & 81.17 & 0.2933 \\
    \Checkmark & \Checkmark &   & \Checkmark &   & 64.64 & 81.49 & 0.2970 \\ 
    \Checkmark & \Checkmark & \Checkmark &   &   & 64.51 & 81.47 & 0.2912 \\ 
    \Checkmark & \Checkmark &   &   & \Checkmark & 65.10 & 80.00 & 0.2972 \\
    \bottomrule
    \end{tabular}}
    \label{tab:ablation}%
\end{table}

\begin{figure}[t]
    \centering
    \subfigure[Low-pass]{
        \includegraphics[width=0.18\linewidth]{iclr2023/pic/low_dependency.pdf}
    }
    \subfigure[High-pass]{
        \includegraphics[width=0.18\linewidth]{iclr2023/pic/high_dependency.pdf}
    }
    \subfigure[Band-pass]{
        \includegraphics[width=0.18\linewidth]{iclr2023/pic/band_dependency.pdf}
    }
    \subfigure[Band-rejection]{
        \includegraphics[width=0.18\linewidth]{iclr2023/pic/rej_dependency.pdf}
    }
    \subfigure[Comb]{
        \includegraphics[width=0.18\linewidth]{iclr2023/pic/comb_dependency.pdf}
    }
    \caption{The dependency of eigenvalues on synthetic graphs.}
    \label{fig:dependece_synthetic}
\end{figure}

\begin{figure}[t]
    \centering
    \subfigure[Dependency of Citeseer]{
        \includegraphics[width=0.23\linewidth]{iclr2023/pic/citeseer_dependency.pdf}
    }
    \subfigure[Filter of Citeseer]{
        \label{fig:filter_of_citeseer}
        \includegraphics[width=0.23\linewidth]{iclr2023/pic/citeseer.pdf}
    }
    \subfigure[Dependency of Squirrel]{
        \includegraphics[width=0.23\linewidth]{iclr2023/pic/squirrel_dependency.pdf}
    }
    \subfigure[Filter of Squirrel]{
        \label{fig:filter_of_squirrel}
        \includegraphics[width=0.23\linewidth]{iclr2023/pic/squirrel.pdf}
    }
    \caption{The dependency and learned filters of heterophilic and homophilic datasets.}
    \label{fig:dependece_node}
\end{figure}

We perform ablation studies on two node-level datasets and one graph-level dataset to evaluate the effectiveness of each component. The results are shown in Table \ref{tab:ablation}.
The top three lines show the effect of the encoder, \ie, eigenvalue encoding (EE) and self-attention. It can be seen that EE is more important on Squirrel than on Citeseer. The reason is that the spectral filter of Squirrel is more difficult to learn. Therefore, the model needs the encoding to learn better representations. The attention module consistently improves performance by capturing the dependency among eigenvalues.

The bottom three lines verify the performance of graph filters at different scales.
We can see that in the easy task, \eg, Citeseer, the Small and Medium models have similar performance, but the Large model causes serious overfitting.
In the hard task, \eg, Squirrel and MolPCBA, the Large model is slightly better than the Medium model but outperforms the Small model a lot, implying that adding the number of parameters can boost the performance.
In summary, it is important to consider the difficulty of tasks when selecting models.

\begin{figure}[H]
    \centering
    \subfigure[dependency of $\hat{\mS}_{1}$]{
        \includegraphics[width=0.23\linewidth]{iclr2023/pic/zinc_head1.pdf}
    }
    \subfigure[Filter of $\hat{\mS}_{1}$]{
        \includegraphics[width=0.23\linewidth]{iclr2023/pic/zinc_filter1.pdf}
    }
    \subfigure[dependency of $\hat{\mS}_{2}$]{
        \includegraphics[width=0.23\linewidth]{iclr2023/pic/zinc_head2.pdf}
    }
    \subfigure[Filter of $\hat{\mS}_{2}$]{
        \includegraphics[width=0.23\linewidth]{iclr2023/pic/zinc_filter2.pdf}
    }
    \caption{The dependency and basic filters of ZINC dataset.}
    \label{fig:dependency_zinc}
\end{figure}

\subsection{Visualizations}
We now investigate the dependency of eigenvalues and filters learned by Specformer. 
% Considering the number of eigenvalues, it is meaningless to visualize the self-attention matrix directly.
To make the dependency clearer, we first quantize the self-attention weight matrix by grouping the eigenvalues into three frequency bands: Low $\in [0, \frac{2}{3})$, Medium $\in [\frac{2}{3}, \frac{4}{3})$, and High $\in [\frac{4}{3}, 2]$.
We then compute the quantized dependency.
More details are given in Appendix \ref{appendix: condense}.

The results are shown in Figures \ref{fig:dependece_synthetic}, \ref{fig:dependece_node}, and \ref{fig:dependency_zinc}, from which we have some interesting observations.
(1) Similar dependency patterns can be learned on different graphs.
In low-pass filtering, \eg, Citeseer and Low-pass, all frequency bands tend to use the low-frequency information.
While, in the band-related filtering, \eg, Squirrel, Band-pass, and Band-rejection, the low- and high-frequency highly depend on the medium-frequency, and the situation of the medium-frequency is opposite.
(2) The more difficult the task, the less obvious the dependency.
On Comb and ZINC, the dependency of eigenvalues is inconspicuous.
% This motivates us to consider more information to capture the dependency of challenging graphs.
(3) On graph-level datasets, the decoder can learn different filters.
Figure \ref{fig:dependency_zinc} shows two basic filters. It can be seen that $\hat{\mS}_{1}$ and $\hat{\mS}_{2}$ have different dependencies and patterns, which are different from node-level tasks, where only one filter is needed.
The finding suggests that these graph-level tasks are more difficult than node-level tasks and are still challenging for spectral GNNs.

==> sections/intro.tex <==
\section{Introduction}\label{sec:intro}

Graph neural networks (GNNs), firstly proposed in \citep{scarselli2008graph}, become increasingly popular in the field of machine learning due to their empirical successes. 
Depending on how the graph signals (or features) are leveraged, GNNs can be roughly categorized into two classes, namely spatial GNNs and spectral GNNs.
Spatial GNNs often adopt a message passing framework \citep{gilmer2017neural,battaglia2018relational}, which learns useful graph representations via propagating local information on graphs.
Spectral GNNs \citep{bruna2013spectral,ChebyNet} instead perform graph convolutions via spectral filters (\ie, filters applied to the spectrum of the graph Laplacian), which can learn to capture non-local dependencies in graph signals.
Although spatial GNNs have achieved impressive performances in many domains, spectral GNNs are somewhat under-explored.

% Recently, graph spectrum based methods received growing attention~\cite{SGC, GNN-LF, FAGCN, robust, Spec-GN}, especially spectral GNNs.
% Spectral GNNs leverage the graph spectrums to design convolutions in the spectral domain, which was shown to have great potential in graph-related tasks \cite{GSP1, GSP2}.
% % Built on top of Graph Signal Processing (GSP) \cite{GSP1}, spectral GNNs can be summarized as three steps: first transforming node features into the spectral domain through the graph Fourier transform, then applying a filter to scale the spectrum of features, and finally inverting the graph Fourier transform to yield new features.
% The design of graph filters is an essential part of spectral GNNs.
% Generally, a good graph filter should utilize the graph spectrum properly to preserve informative frequency components and filter out noise, thus benefiting the performance.
% For example, FAGCN \cite{FAGCN} balances the low-frequency and high-frequency information in the graph spectrum to design an adaptive filter,
% polynomial GNNs \cite{ChebyNet, GPR-GNN, BernNet, Jacobi} combine eigenvalues of different orders to simulate arbitrary filters,
% and LanczosNet \cite{LanczosNet} uses short-range and long-range spectrum information to design a multi-scale graph filter.
There are a few reasons why spectral GNNs have not been able to catch up.
First, most existing spectral filters are essentially scalar-to-scalar functions.
In particular, they take a single eigenvalue as input and apply the same filter to all eigenvalues.
This filtering mechanism could ignore the rich information embedded in the spectrum, \ie, the set of eigenvalues.
For example, we know from the spectral graph theory that the algebraic multiplicity of the eigenvalue $0$ tells us the number of connected components in the graph.
However, such information can not be captured by scalar-to-scalar filters.
% which significantly restricts their ability to learn the optimal filter.
Second, the spectral filters are often approximated via fixed-order (or truncated) orthonormal bases, \eg, Chebyshev polynomials \citep{ChebyNet, Chebyshev2} and graph wavelets \citep{hammond2011wavelets,xu2019graph}, in order to avoid the costly spectral decomposition of the graph Laplacian.
Although the orthonormality is a nice property, this truncated approximation is less expressive and may severely limit the graph representation learning. 

% \emph{How to effectively leverage the spectrum of graph Laplacian to design graph filters?}
% This is a fundamental question since the spectrum directly affects the learning ability of graph filters.
% Because the success of deep learning is attributed to the powerful representation learning capability, it is promising to encode spectrum information into representations and use it in graph filters.
% \emph{How to learn meaningful representations of the spectrum?}
% A well-informed answer can yield profound insights into the design of graph filters and deepen our understanding of graph spectrums.

Therefore, in order to improve spectral GNNs, it is natural to ask: \emph{how can we build expressive spectral filters that can effectively leverage the spectrum of graph Laplacian}? 
% Intuitively, the representations of the graph spectrum should contain information from two perspectives: position information and set information.
% First, eigenvalues indicate the positions on the graph spectrum \cite{SAN}.
% Therefore, the representations of the graph spectrum should include the absolute positional information of eigenvalues so that the graph filters can learn how to scale the input signals by shifting the positions.
To answer this question, we first note that eigenvalues of graph Laplacian represent the frequency, \ie, total variation of the corresponding eigenvectors.
The magnitudes of frequencies thus convey rich information.
Moreover, the relative difference between two eigenvalues also reflects important frequency information, \eg, the spectral gap.
% Hence, a good spectrum representation should also express the relative positional information.
% Second, eigenvalues are a set of scalars with compact connections.
% It is important to consider the set attribute when learning the  representations of spectrums.
% For example, previous polynomial filters, treating the eigenvalues individually, are all univariate polynomials, and the theoretical learning ability is far from that of multivariate polynomials.
% When learning the representations of eigenvalues, we should not only consider the dependency among them but also preserve some important property, e.g., permutation equivariant.
% First, most graph filters are scalar-to-scalar functions. They apply the filtering functions to each eigenvalue individually and ignore the complex dependency between different eigenvalues.
% For example, polynomial filters \cite{ChebyNet, GPR-GNN, BernNet, Chebyshev2, Jacobi, EvenNet} combine eigenvalues of different orders to simulate arbitrary filters.
% Without considering the dependency, existing polynomials are all univariate, and the theoretical learning ability is far from that of multivariate polynomials.
% \lele{[Do you mean the filtering functions can all be written as a single variable polynomial? It's unclear to me what ``they'' refers to and what ``polynomials of a variable'' means]} 
% Moreover, eigenvalues are a set of scalars with rich semantic information describing the global structures of graphs \cite{SAN}. Scalar-to-scalar functions lack the modeling of eigenvalues and cannot fully exploit the implicit semantic information.
% Second, existing graph filters are difficult to adapt to different graphs.
% Let us still take the polynomial filters as an example. The filtering functions of polynomials are learned on the spectrums of the training graphs and do not change adaptively when transferred to the testing graphs.
% The parameters of polynomials are trained in the seen \lele{[training?]} graphs and would not change adaptively when transferred to the unseen \lele{[testing?]} graphs.
% However, the eigenvalues of different graphs may vary significantly. The high-order terms of polynomials may be greatly affected by a slight eigenvalue shift \cite{ARMA}.
% Finally, the learned graph filters will be far away from the optimal one.
% Moreover, to fit the optimal filter more accurately, polynomial filters need to increase the degree, resulting in poor stability and ill-posed optimization problems.
% Some methods \cite{spctralCNN, LanczosNet} use truncated eigenvalues, e.g., top-$K$ eigenvalues, to enhance learning ability. However, this truncation will lose important frequency information, e.g., band- and high-frequency information, and limits the application of these methods.
To capture both magnitudes of frequency and relative frequency, we propose a Transformer \citep{vaswani2017attention} based set-to-set spectral filter, termed \emph{Specformer}.
Our Specformer first encodes the range of eigenvalues via positional embedding and then exploits the self-attention mechanism to learn relative information from the set of eigenvalues.
% spectrum representations with rich positional and set information, in this paper, we propose a novel set-to-set graph filter, termed \emph{Specformer}.
% The focal component of Specformer is a spectral domain Transformer block, which uses an elaborate eigenvalue encoding function and the self-attention mechanism to capture the positional information and fine-grained dependency of eigenvalues, respectively.
% Due to the high nonlinearity of Transformer, the scalar eigenvalues can be transformed into meaningful representations.
Relying on the learned representations of eigenvalues, we also design a decoder with a bank of learnable bases.
Finally, by combining these bases, Specformer can construct a permutation-equivariant and non-local graph convolution.
% The superior learning ability of Specformer is first demonstrated by a synthetic filtering test and further supported by experiments on real-world datasets.
% The synthetic experiments clearly show that Specformer can fit the optimal filter well, even in several narrow bands where the polynomial filters perform poorly.
% Specformer also achieves state-of-the-art performance on most real-world graph-related tasks, including node classification, graph classification, and regression.
% Additionally, we visualize the learned self-attention matrix and find that the dependency patterns of eigenvalues can be transferred across graphs, which could potentially inspire more work to discover the relationship between graph spectrum and GNNs.
In summary, our contributions are as follows:
% \begin{itemize}[leftmargin=*]
\begin{itemize}
% \item To the best of our knowledge, we are the first to consider learning meaningful representations of graph spectrums to produce high-quality graph filters.
\item We propose a novel Transformer-based set-to-set spectral filter along with learnable bases, called Specformer, which effectively captures both magnitudes and relative differences of all eigenvalues of the graph Laplacian.
\item We show that Specformer is permutation equivariant and can perform non-local graph convolutions, which is non-trivial to achieve in many spatial GNNs.
\item Experiments on synthetic datasets show that Specformer learns to better recover the given spectral filters than other spectral GNNs.
\item Extensive experiments on various node-level and graph-level benchmarks demonstrate that Specformer outperforms state-of-the-art GNNs and learns meaningful spectrum patterns.
\end{itemize}



==> sections/method.tex <==
\begin{wrapfigure}[18]{r}{0.35\linewidth}
    % \vspace{-40pt}
    \centering
    \includegraphics[width=\linewidth]{pic/model.pdf}
    \vspace{-18pt}
    \caption{Illustration of the proposed Specformer.}
    % \lele{In the figure, there is a block called ``graph convolutional''. Do you mean ``graph convolution''?}
    \label{fig:model}
\end{wrapfigure}

\section{Specformer}
In this section, we introduce our Specformer model. Fig. \ref{fig:model} illustrates the model architecture.
We first explain how we encode the eigenvalues and use Transformer to capture their dependencies to yield useful representations.
Then we turn to the decoder, which learns new eigenvalues from the representations and reconstructs the graph Laplacian matrix for graph convolution.
Finally, we discuss the relationship between our Specformer and other methods, including MPNNs, polynomial GNNs, and graph Transformers.

% \subsection{Spectral Graph Filter}
% The spectral graph filter of Specformer contains two parts: encoding and decoding.
% In the encoding part, an eigenvalue encoding function 

% a vanilla Transformer is used as an encoder to learn the dependency of eigenvalues.
% In the decoding part, a multilayer perceptron (FFN) is used to decode a set of eigenvalues as the new graph spectrum.

\subsection{Eigenvalue Encoding}
We design a powerful set-to-set spectral filter using Transformer to leverage both magnitudes and relative differences of all eigenvalues.
However, the expressiveness of self-attention will be restricted heavily if we directly use the scalar eigenvalues to calculate the attention maps.
Therefore, it is important to find a suitable function, $\rho(\lambda): \R^{1} \rightarrow \R^{d}$, to map each eigenvalue from a scalar to a meaningful vector. 
We use an eigenvalue encoding function as follows.
\begin{equation}
\begin{split}
\rho(\lambda, 2i)&=\sin (\epsilon \lambda / 10000^{2i/d}), \\
\rho(\lambda, 2i+1)&=\cos (\epsilon \lambda / 10000^{2i/d}),
\end{split}
\label{eq: EE}
\end{equation}
where $i$ is the dimension of the representations and $\epsilon$ is a hyperparameter.
The benefits of $\rho(\lambda)$ are three-fold:
(1) It can capture the relative frequency shifts of eigenvalues and provides high-dimension vector representations.
(2) It has the wavelengths from $2\pi$ to $10000 \cdot 2\pi$, which forms a multi-scale representation for eigenvalues.
(3) It can control the influence of $\lambda$ by adjusting the value of $\epsilon$.

The choice of $\epsilon$ is crucial because we find that only the first few dimensions of $\rho(\lambda)$ can distinguish different eigenvalues if we simply set $\epsilon=1$.
The reason is that eigenvalues lie in the range $[0, 2]$, and the value of $\lambda/10000^{2i/d}$ will change slightly when $i$ becomes larger.
Therefore, it is important to assign a large value of $\epsilon$ to enlarge the influence of $\lambda$.
Experiments can be seen in Appendix \ref{appendix: EE}.

Notably, although the eigenvalue encoding (EE) is similar to the positional encoding (PE) of Transformer, they act quite differently.
PE describes the information of discrete positions in the spatial domain.
While EE represents the information of continuous eigenvalues in the spectral domain.
Applying PE to the spatial positions (\ie, indices) of eigenvalues will destroy the permutation equivariance property, thereby impairing the learning ability.

% We choose the positional encoding (PE) function of Transformer \cite{transformer} as the mapping function:
% \begin{equation}
% \begin{split}
% \text{PE}(pos, 2i)   &= \sin (pos / 10000^{2i/d}), \\
% \text{PE}(pos, 2i+1) &= \cos (pos / 10000^{2i/d}),
% \end{split}
% \label{eq: PE}
% \end{equation}

% However, we find that only the first few dimensions of PE can distinguish different eigenvalues if we directly replace $pos$ with $\lambda$.
% The reason is that eigenvalues lie in the range $[0, 2]$, and the value of $\lambda/10000^{2i/d}$ will change slightly when $i$ becomes larger.
% Therefore, we multiply each eigenvalue with a constant $\epsilon$ to enlarge its influence, which can be formally characterized as:
% \begin{equation}
% \begin{split}
% \rho(\lambda, 2i)&=\sin (\epsilon \lambda / 10000^{2i/d}), \\
% \rho(\lambda, 2i+1)&=\cos (\epsilon \lambda / 10000^{2i/d}).
% \end{split}
% \end{equation}
% \lele{[Can we directly introduce the expression in (3), rather than first giving expression (2) and then explaining why expression (2) is bad? You can still explain the role of $\epsilon$ and say the standard positional encoding corresponds to the case $\epsilon = 1$. You can then explain why the standard PE is not good.]}

The initial representations of eigenvalues are the concatenation of eigenvalues and their encodings, $\mZ = [\lambda_{1} \| \rho(\lambda_{1}), \cdots, \lambda_{n} \| \rho(\lambda_{n})]^{\top} \in \R^{n \times (d+1)}$.
Then a standard Transformer block is used to learn the dependency between eigenvalues.
We first apply layer normalization (LN) on the representations before feeding them into other sub-layers, \ie, MHA and FFN.
This \emph{pre-norm} trick has been used widely to improve the optimization of Transformer \citep{Graphormer}:
\begin{equation}
\begin{split}
    \tilde{\mZ} &= \text{MHA}(\text{LN}(\mZ)) + \mZ, \\
    \hat{\mZ} &= \text{FFN}(\text{LN}(\tilde{\mZ})) + \tilde{\mZ}.
\end{split}
\end{equation}
% After stacking multiple Transformer blocks, the high nonlinearity of MHA and FFN enables the encoder to learn meaningful representations and prepares for the decoder to generate new eigenvalues.
After stacking multiple Transformer blocks, we obtain the expressive representations of the spectrum.

\subsection{Eigenvalue Decoding}

Based on the representations returned by the encoder, the decoder can learn new eigenvalues for spectral filtering.
Recent studies \citep{Spec-GN, Jacobi} show that assigning each feature dimension a separate spectral filter improves the performance of GNNs.
Motivated by this discovery, our decoder first decodes several bases. 
An FFN is then used to combine these bases to construct the final graph convolution.

\paragraph{Spectral filters.}
In general, the bases should learn to cover different information of the graph signal space as much as possible.
For this purpose, we utilize the multi-head attention mechanism because each head has its own self-attention module.
Specifically, the representations learned by each head will be fed into the decoder to perform spectral filtering to get the new eigenvalues.
\begin{equation}
    \mZ_{m} = \text{Attention}(\mQ\mW^{Q}_{m}, \mK\mW^{K}_{m}, \mV\mW^{V}_{m}), \quad \bm{\lambda}_{m}=\phi(\mZ_{m} \mW_{\lambda}),
\label{eq: decoder}
\end{equation}
where $\mZ_{m}$ denotes the representations learned by the $m$-th heads, and $\phi$ is the activation, \eg, ReLU or Tanh, which is optional.
$\bm{\lambda}_{m} \in \R^{n \times 1}$ is the $m$-th eigenvalues after the spectral filtering.


% To modulate the node features, we need to decode new eigenvalues as the graph filter.
% However, the graph filter will depend on the graph structures and cannot adapt to the data if we only consider the information of eigenvalues, i.e., $Z^{l}$.
% To overcome this issue, we also consider the node representations in the decoding process:
% \begin{equation}
%     \bm{\lambda}^{l}=\phi ([Z^{l} \| X^{l}]W_{\lambda}^{l}),
% \end{equation}
% where $\bm{\lambda}^{l} \in \mathbb{R}^{n \times 1}, X^{l} \in \mathbb{R}^{n \times d}$ indicate the new eigenvalues and node representations in $l$-th layer, respectively. $W_{\lambda}^{l} \in \mathbb{R}^{2d \times 1}$ is the decoding vector and $\phi$ represents some constraints on eigenvalues.

% \paragraph{Constraints on eigenvalues.}
% Recent studies \cite{SGC, BernNet} show that introducing some necessary constraints on the eigenvalues is important for optimizing spectral-based GNNs.
% Here, we use $\rm tanh(\cdot)$ to restrict the absolute values of new eigenvalues, which can limit the range of eigenvalues can be bounded to [-1, 1], even if the model stacks multiple layers.

\paragraph{Learnable bases.} 
After get $M$ filtered eigenvalues, we use a FFN: $\R^{M+1} \rightarrow \R^{d}$ to construct the learnable bases. 
% This combination includes many neural network tricks, such as normalization, activation, etc.
We first reconstruct individual new bases, concatenate them along the channel dimension, and feed them to a FFN as below,
\begin{equation}
    \mS_{m}=\mU \text{diag}(\bm{\lambda}_{m}) \mU^{\top}, \quad \hat{\mS} = \text{FFN}([\mI_{n} || \mS_{1} || \cdots || \mS_{M}]),
\end{equation}
where $\mS_{m} \in \R^{n \times n}$ is the $m$-th new basis and $\hat{\mS} \in \R^{n \times n \times d}$ is the combined version.
Note that our bases here serve similar purpose as those polynomial bases in the literature.
But the way they are combined is learned rather than following certain recursions as in Chebyshev polynomials.
% Moreover, we can mix the learnable basic filters and combinations to build filters of different scales. 

We have three optional ways to leverage this design of new bases.
(1) Shared filters and shared FFN. This model has the least parameters, where the basis $\hat{\mS}$ is shared across all graph convolutional layers.
(2) Shared filters and layer-specific FFN, which compromises between parameters and performance, \eg, $\hat{\mS}^{(l)} = \text{FFN}^{(l)}([\mI_{n} || \mS_{1} || \cdots || \mS_{M}])$ where the superscript $l$ denotes the index of layer.
(3) Layer-specific filters and layer-specific FFN. This model has the most parameters and each layer has its own encoder and decoder, \eg, $\hat{\mS}^{(l)} = \text{FFN}^{(l)}([\mI_{n} || \mS_{1}^{(l)} || \cdots || \mS_{M}^{(l)}])$.
We refer these three models as Specformer-Small, Specformer-Medium, and Specformer-Large.

\subsection{Graph Convolution}

Finally, we assign each feature dimension a separate graph Laplacian matrix based on the learned basis $\hat{\mS}$, which can be written as follows:
% we can \sout{convolute} \lele{convolve $\mS$ with} the node features in the vertical domain \lele{[Is this what you mean?]}
\begin{equation}
    \hat{\mX}^{(l-1)}_{:,i} = \hat{\mS}_{:,:,i} \mX^{(l-1)}_{:,i}, \quad
    \mX^{(l)} =  \sigma \left(\hat{\mX}^{(l-1)} \mW_{x}^{(l-1)} \right) + \mX^{(l-1)},
\label{eq: convolution}
\end{equation}
where $\mX^{(l)}$ is the node representations in the $l$-th layer, $\hat{\mX}^{(l-1)}_{:,i}$ is the $i$-th channel dimension, $\mW_{x}^{(l-1)}$ is the transformation, and $\sigma$ is the activation.
The residual connection is an optional choice.
By stacking multiple graph convolutional layers, Specformer can effectively learn node representations.

\subsection{Key Properties Compared to Related Models}

\paragraph{Specformer \textit{v.s.} Polynomial GNNs.} Specformer replaces the fixed bases of polynomials, \eg, $\lambda, \lambda^{2}, \cdots, \lambda^{k}$, with learnable bases, which has two major advantages:
(1) Universality. Polynomial GNNs are the special cases of Specformer because the learnable bases can approximate any polynomials.
(2) Flexibility. Polynomial GNNs are designed to learn a shared function for all eigenvalues
% falling into a dilemma between precision and stability. 
whereas Specformer can learn eigenvalue-specific functions, thus being more flexible.

% are sensitive to small disturbances because of the high-order bases. JacobiConv \cite{Jacobi} proposes a coefficient decomposition trick to alleviate this issue. Specformer 

\vspace{-7pt}
\paragraph{Specformer \textit{v.s.} MPNNs.} MPNNs aggregate the local information from neighborhood one hop per layer. This localization capability enables MPNNs with high computational efficiency but weakens the ability in capturing the global information.
Specformer is inherently non-local due to the use of (often dense) eigenvectors. 
The learned graph Laplacian $\mU G_{\theta} \mU^{\top} = \theta_{1}\vu_{1}\vu_{1}^{\top} + \cdots + \theta_{n}\vu_{n}\vu_{n}^{\top}$. 
Because $\vu_{i}$ is a eigenvector, $\vu_{i}\vu_{i}^{\top}$ constructs a fully-connected graph. 
Therefore, our Specformer can break the localization of MPNNs and leverage global information.
% With proper weights of $G_{\theta}$, the graph can break the localization of MPNNs and leverage global information.

\vspace{-7pt}
\paragraph{Specformer \textit{v.s.} Graph Transformers.}
Graphormer \citep{Graphormer} has shown that graph Transformer can perform well on graph-level tasks.
However, existing graph Transformers do not show competitiveness in the node-level tasks, \eg, node classification.
Recent studies \citep{over3, over1, over2} provide some evidence for this phenomenon. They show that Transformer is essentially a low-pass filter. Therefore, graph Transformers cannot handle the complex node label distribution, \eg, homophilic and heterophilic.
On the contrary, as we will see in the experiment section, Specformer can learn arbitrary bases for graph convolution and perform well on both node-level and graph-level tasks.

% \vspace{-7pt}
% \paragraph{Theoretical Results.}
Besides the above advantages, we show that our Specformer has the following theoretical properties.

\begin{proposition}
\label{propos: pe}
Specformer is permutation equivariant.
\end{proposition}

\begin{proposition}
\label{propos: approximate}
Specformer can approximate any univariate and multivariate continuous functions.
\end{proposition}

% \vspace{-10pt}
% \begin{proof}
% See Appendix \ref{appendix: univariate} for proof.
% \end{proof}
% \vspace{-5pt}

% \begin{proposition}
% \label{propos: multivariate}
% Specformer can approximate any  continuous functions.
% \end{proposition}

% \vspace{-10pt}
% \begin{proof}
% See Appendix \ref{appendix: multivariate} for proof.
% \end{proof}
% \vspace{-15pt}
% \renjie{Comment here that Specformer can approximate any eigenvalue and any set of eigenvalues!}

% \textcolor{blue}{
Proposition \ref{propos: pe} shows that Specformer can learn permutation-equivariant node representations.
Proposition \ref{propos: approximate} states that Specformer is more expressive than other graph filters.
First, the ability to approximate any univariate functions generalizes existing scalar-to-scalar filters.
Besides, Specformer can handle multiple eigenvalues and learn multivariate functions, so it can approximate a broader range of filter functions than scalar-to-scalar filters.
All proofs are provided in Appendix \ref{appendix: theoretical}
% }

% \sout{Because eigenvalues are in the interval $[0, 2]$, Specformer can approximate any continuous functions acting on a single eigenvalue or a set of eigenvalues.}

\paragraph{Complexity.}
Specformer has two parts of computation: spectral decomposition and forward process.
Spectral decomposition is pre-computed and has the complexity of $\mathcal{O}(n^3)$.
The forward complexity has three parts: Transformer, learnable bases, and graph convolution.
Their corresponding complexities are $\mathcal{O}(n^{2}d + nd^{2})$, $\mathcal{O}(Mn^{2})$ and $\mathcal{O}(Lnd)$, respectively, where $n, M, L$ represent the number of nodes, filters, and layers, and $d$ is the hidden dimension.
The overall forward complexity is $\mathcal{O}(n^{2}(d+M) + nd(L+d))$.
The overall complexity of Specformer is the sum of the forward complexity and the decomposition complexity amortized over the number of uses in training and inference, rather than a simple summation of the two.
See Appendix \ref{appendix: overhead} for more discussion.

\vspace{-7pt}
\paragraph{Scalability.} When applying Specformer to large graphs, one can use the Sparse Generalized Eigenvalue (SGE) algorithms \citep{SGE1} to calculate $q$ eigenvalues and eigenvectors, in which case the forward complexity will reduce to $(q^{2}(d+M) + nd(L+d))$.
\vspace{-5pt}

==> sections/related.tex <==
\section{Related Work}
Existing GNNs can be roughly divided into two categories: spatial and spectral GNNs. 

\vspace{-10pt}
\paragraph{Spatial GNNs.}
Spatial GNNs like GAT \citep{GAT} and MPNN \citep{gilmer2017neural} leverage message passing to aggregate local information from neighborhoods.
By stacking multiple layers, spatial GNNs can possibly learn long-range dependencies but suffer from over-smoothing \citep{over-smoothing} and over-squashing \citep{over-squashing}.
Therefore, how to balance local and global information is an important research topic for spatial GNNs.
We refer readers to \citep{survey1,survey2,liao2021deep} for a more detailed discussion about spatial GNNs.

\vspace{-10pt}
\paragraph{Spectral GNNs.}
Spectral GNNs \citep{GSP1, GSP2, SGC, GNN-LF, FAGCN, robust, Spec-GN} leverage the spectrum of graph Laplacian to perform convolutions in the spectral domain.
% It has shown great potential in graph-related tasks \citep{GSP1, GSP2}.
% Built on top of Graph Signal Processing (GSP) \cite{GSP1}, spectral GNNs can be summarized as three steps: first transforming node features into the spectral domain through the graph Fourier transform, then applying a filter to scale the spectrum of features, and finally inverting the graph Fourier transform to yield new features.
% The design of graph filters is an essential part of spectral GNNs.
% Generally, a good graph filter should utilize the graph spectrum properly to preserve informative frequency components and filter out noise, thus benefiting the performance.
% Most spectral GNNs focus on the design of efficient spectral filters.
A popular subclass of spectral GNNs leverages different kinds of orthogonal polynomials to approximate arbitrary filters, including Monomial \citep{GPR-GNN}, Chebyshev \citep{ChebyNet, GCN, Chebyshev2}, Bernstein \citep{BernNet}, and Jacobi \citep{Jacobi}.
Relying on the diagonalization of symmetric matrices, they avoid direct spectral decomposition and guarantee localization.
However, all such polynomial filters are scalar-to-scalar functions, and the bases are pre-defined, which limits their expressiveness.
% For example, polynomial GNNs \citep{ChebyNet, GPR-GNN, BernNet, Jacobi} combine eigenvalues of different orders to simulate arbitrary filters,
% and LanczosNet \cite{LanczosNet} uses short-range and long-range spectrum information to design a multi-scale graph filter.
% FAGCN \citep{FAGCN} balances the low-frequency and high-frequency information in the spectrum to design an adaptive filter.
Another subclass requires either full or partial spectral decomposition, such as SpectralCNN \citep{spctralCNN} and LanczosNet \citep{LanczosNet}.
They parameterize the spectral filters by neural networks, thus being more expressive than truncated polynomials. However, such spectral filters are still limited as they do not capture the dependencies among multiple eigenvalues.
% SpectralCNN directly treats the graph spectrum as the parameters of neural networks and updates them through gradient descent. 
% LanczosNet designs a multi-scale learnable filter to encode the short-range and long-range information. However, they only use partial spectrum information, i.e., top-$K$ eigenvalues.

\vspace{-10pt}
\paragraph{Graph Transformer.} 
Transformers and GNNs are closely relevant since the attention weights of Transformer can be seen as a weighted adjacency matrix of a fully connected graph.
% which breaks the localization property of GNNs and shows great potential for graph-related tasks. 
Graph Transformers \citet{GT} combine both and have gained popularity recently. 
Graphormer \citep{Graphormer}, SAN \citep{SAN}, and GPS \citep{GPS} design powerful positional and structural embeddings to further improve their expressive power.
Graph Transformers still belong to spatial GNNs, although the high-cost self-attention is non-local.
The limitation of spatial attention compared to spectral attention has been discussed in \citep{over3}.
% Although significant progress has been made, existing graph Transformers are designed only for graph-level tasks. 
% None of them show competitiveness on node-level tasks.
